A Comprehensive Study on Colorectal Polyp Segmentation with ResUNet++, Conditional Random Field and Test-Time Augmentation

Colonoscopy is considered the gold standard for detection of colorectal cancer and its precursors. Existing examination methods are, however, hampered by high overall miss-rate, and many abnormalities are left undetected. Computer-Aided Diagnosis systems based on advanced machine learning algorithms are touted as a game-changer that can identify regions in the colon overlooked by the physicians during endoscopic examinations, and help detect and characterize lesions. In previous work, we have proposed the ResUNet++ architecture and demonstrated that it produces more efficient results compared with its counterparts U-Net and ResUNet. In this paper, we demonstrate that further improvements to the overall prediction performance of the ResUNet++ architecture can be achieved by using conditional random field and test-time augmentation. We have performed extensive evaluations and validated the improvements using six publicly available datasets: Kvasir-SEG, CVC-ClinicDB, CVC-ColonDB, ETIS-Larib Polyp DB, ASU-Mayo Clinic Colonoscopy Video Database, and CVC-VideoClinicDB. Moreover, we compare our proposed architecture and resulting model with other State-of-the-art methods. To explore the generalization capability of ResUNet++ on different publicly available polyp datasets, so that it could be used in a real-world setting, we performed an extensive cross-dataset evaluation. The experimental results show that applying CRF and TTA improves the performance on various polyp segmentation datasets both on the same dataset and cross-dataset.

==> author.tex <==
% \author{\IEEEauthorblockN{Debesh Jha\IEEEauthorrefmark{1}\IEEEauthorrefmark{3}, Pia H. Smedsrud\IEEEauthorrefmark{1}\IEEEauthorrefmark{2}\IEEEauthorrefmark{4}, Dag Johansen\IEEEauthorrefmark{3}, \\ Thomas de Lange\IEEEauthorrefmark{2}\IEEEauthorrefmark{6}\IEEEauthorrefmark{7}, 
% H{\aa}vard D. Johansen\IEEEauthorrefmark{3}, P{\aa}l Halvorsen\IEEEauthorrefmark{1}\IEEEauthorrefmark{5}, Michael A. Riegler\IEEEauthorrefmark{1}\IEEEauthorrefmark{4}
% }
% \vspace{2mm}
% \IEEEauthorblockA{\IEEEauthorrefmark{1}SimulaMet, Norway \ \ \ \ \ \
% \IEEEauthorrefmark{2}Augere Medical AS, Norway \ \ \ \ \ \
% \IEEEauthorrefmark{3}UiT The Arctic University of Norway, Norway \\ 
% \IEEEauthorrefmark{4}University of Oslo, Norway\ \ \ \ \ \ \
% \IEEEauthorrefmark{5}Oslo Metropolitan University, Norway\\
% \IEEEauthorrefmark{6}Sahlgrenska University Hospital, Mölndal, Sweden\ \ \ \ \ \ \
% \IEEEauthorrefmark{7}Bærum Hospital, Vestre Viken, Norway\\
% Email: {debesh@simula.no}}}



==> cutout.tex <==
Colonoscopy is only the procedure for discovering and removing adenomatous polyp. Among the primary health problem of contemporary society is cancer, with \ac{CRC} being the most prevailing strain globally~\cite{haggar2009colorectal}. Early detection of \ac{CRC} is crucial for improving the survival rate.  \par  


%----not cited int the paper%-----------------------
@article{haggar2009colorectal,
  title={Colorectal cancer epidemiology: incidence, mortality, survival, and risk factors},
  author={Haggar, Fatima A and Boushey, Robin P},
  journal={Clinics in colon and rectal surgery},
  volume={22},
  number={04},
  pages={191--197},
  year={2009}
}

@article{holme2013flexible,
  title={Flexible sigmoidoscopy versus faecal occult blood testing for colorectal cancer screening in asymptomatic individuals},
  author={Holme, {\O}yvind and Bretthauer, Michael and Fretheim, Atle and Odgaard-Jensen, Jan and Hoff, Geir},
  journal={Cochrane Database of Systematic Reviews},
  number={9},
  year={2013}
}

@article{geetha2017heuristic,
author = {K, Geetha and C, Rajan},
doi = {10.22034/APJCP.2017.18.6.1681},
file = {::},
issn = {2476-762X},
journal = {Asian Pacific journal of cancer prevention : APJCP},
keywords = {Colon cancer,Colonoscopy,Polyps,Segmentation,Video Capsule Endoscopy,binary pattern},
number = {6},
pages = {1681--1688},
pmid = {28670889},
title = {{Heuristic Classifier for Observe Accuracy of Cancer Polyp Using Video Capsule Endoscopy}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/28670889},
volume = {18},
year = {2017}
}

@article{quintero2012progress,
  title={Progress and challenges in colorectal cancer screening},
  author={Quintero, Enrique and Hassan, Cesare and Senore, Carlo and Saito, Yutaka},
  journal={Gastroenterology research and practice},
  volume={2012},
  year={2012}
}

@article{rex2002rationale,
  title={Rationale for colonoscopy screening and estimated effectiveness in clinical practice.},
  author={Rex, Douglas K},
  journal={Gastrointestinal endoscopy clinics of North America},
  volume={12},
  number={1},
  pages={65--75},
  year={2002}
}


@article{rex2002quality,
  title={Quality in the technical performance of colonoscopy and the continuous quality improvement process for colonoscopy: recommendations of the US Multi-Society Task Force on Colorectal Cancer},
  author={Rex, Douglas K and others},
  journal={The American journal of gastroenterology},
  volume={97},
  number={6},
  pages={1296},
  year={2002}
}

@inproceedings{pogorelov2017holistic,
  title={A holistic multimedia system for gastrointestinal tract disease detection},
  author={Pogorelov, Konstantin and others},
  booktitle={Proceedings of the 8th ACM on Multimedia Systems Conference},
  pages={112--123},
  year={2017}
  }
@article{pabby2005analysis,
  title={Analysis of colorectal cancer occurrence during surveillance colonoscopy in the dietary Polyp Prevention Trial},
  author={Pabby, Ajay and others},
  journal={Gastrointestinal endoscopy},
  volume={61},
  number={3},
  pages={385--391},
  year={2005}
}


@article{wang2015polyp,
  title={Polyp-alert: Near real-time feedback during colonoscopy},
  author={Wang, Yi and Tavanapong, Wallapak and Wong, Johnny and Oh, Jung Hwan and De Groen, Piet C},
  journal={International Journal of Computer methods and programs in biomedicine},
  volume={120},
  number={3},
  pages={164--179},
  year={2015}
}

@article{gkolfakis2017new,
  title={New endoscopes and add-on devices to improve colonoscopy performance},
  author={Gkolfakis, Paraskevas and Tziatzios, Georgios and Dimitriadis, George D and Triantafyllou, Konstantinos},
  journal={World journal of gastroenterology},
  volume={23},
  number={21},
  pages={3784},
  year={2017}
}
@article{mori2018real,
  title={Real-time use of artificial intelligence in identification of diminutive polyps during colonoscopy: a prospective study},
  author={Mori, Yuichi others},
  journal={Annals of internal medicine},
  volume={169},
  number={6},
  pages={357--366},
  year={2018}
}

@inproceedings{brandao2017fully,
  title={Fully convolutional neural networks for polyp segmentation in colonoscopy},
  author={Brandao, Patrick and others},
  booktitle={Medical Imaging 2017: Computer-Aided Diagnosis},
  volume={10134},
  pages={101340F},
  year={2017}
}

@incollection{zhou2018unet++,
  title={Unet++: A nested u-net architecture for medical image segmentation},
  author={Zhou, Zongwei and Siddiquee, Md Mahfuzur Rahman and Tajbakhsh, Nima and Liang, Jianming},
  booktitle={Deep Learning in Medical Image Analysis and Multimodal Learning for Clinical Decision Support},
  pages={3--11},
  year={2018}
}


%This is because different factors can affect the results on the particular dataset (for example, size and ratio of training, validation, and testing dataset). The optimal parameter for the model on one dataset does not necessarily perform well with all other datasets and is sometimes prone to over-fitting. Therefore, we suggest the use of cross-dataset evaluation for measuring the performance of future models.  

%Images, for instance, depict incomplete polyps, polyps partially covered with stool, bubbles, turbid, and other intestinal content. Additional challenges in the images are variations in color, light, angle of the cameras, superfluous information, varying morphology, and instrument over polyp frame, and bowel-quality during colonoscopy. All of these can affect the overall performance of a \ac{DL} model. 



%(vii) in some cases, the appearance, and structures of the non-polyp tissue (mucous, presence of stool in some portion of the polyp) in the input polyp frame are similar to that of polyp tissue,

% Thus, the proposed model can be the baseline for other researchers for the evaluation of their approach on the same dataset close to real world requirements and for cross-dataset. 

% signifance of video frame?

%why all the works are not comapred?
%In such cases, all the methods are trained on the same training set and by definition evaluated on the common test subsets using the same set of metrics. Furthermore, as the evaluation is performed at the same time, it can provide a useful snapshot of the current state-of-the-art and reference for further development.

==> etis_larib_and_ColonDB.tex <==

\begin{table}[t]
 \caption{The table shows additional experimental results for the cross-data evaluation to achieve generalization goal. For training the models, ETIS-Larib dataset is used, and for testing the models, we have used CVC-356, CVC-968, and CVC-12K.}
    \label{table:results2}
   \def\arraystretch{1.1}
    \setlength\tabcolsep{5pt}
    \par\bigskip
    \centering
        \resizebox{\columnwidth}{!}{%
           \begin{tabular}{ l c c c c } 
                \bottomrule
                Method & DICE & IoU & Recall & Precision\\ 
                  \toprule
                \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-356}} \\
              \bottomrule
                \textbf{ResUNet++}& 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline
                {ResUNet++ CRF} & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline
                 {ResUNet++ TTA} & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline
                 {ResUNet++ CRF + TTA} & 0.0000  & 0.0000 & 0.0000 & 0.0000\\ % \hline
                \toprule
                \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-612}}\\
              \bottomrule
              \textbf{ResUNet++}& 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline  
              {ResUNet++ + CRF} & 0.0000 & 0.0000  & 0.0000 & 0.0000\\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  & 0.0000 & 0.0000\\ % \hline
              {ResUNet++ + TTA + CRF}& 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline
                \toprule  
             \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-968}} \\
              \bottomrule
              \textbf{ResUNet++} & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline  
              {ResUNet++ + CRF} & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  &  0.0000 & 0.0000\\ % \hline
              {ResUNet++ + TTA + CRF}& 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline
                \toprule  
                \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-12K}} \\
              \bottomrule
              {ResUNet++}& 0.0000 & 0.0000 & 0.0000  & 0.0000 \\ % \hline  
              {ResUNet++ + CRF} & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline
              {ResUNet++ + TTA + CRF} & 0.0000 & 0.0000 & 0.0000  & 0.0000 \\ % \hline
                \toprule 
             \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = Kvasir-SEG}} \\
              \bottomrule
              ResUNet++ &  0.0000 & 0.0000  & 0.0000  & 0.0000 \\ % \hline  
              {ResUNet++ + CRF}& 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline
              {ResUNet++ + TTA + CRF} & 0.0000  & 0.0000 & 0.0000  & 0.0000 \\ % \hline
                \toprule 
            \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = Colon-DB}} \\
              \bottomrule
              ResUNet++ &  0.0000 & 0.0000  & 0.0000  & 0.0000 \\ % \hline  
              {ResUNet++ + CRF}& 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline
              {ResUNet++ + TTA + CRF} & 0.0000  & 0.0000 & 0.0000  & 0.0000 \\ % \hline
                \toprule 
\end{tabular}}
\end{table}						


\begin{table}[t]
 \caption{The table shows additional experimental results for the cross-data evaluation to achieve generalization goal. For training the models, Colon-DB dataset is used, and for testing the models, we have used CVC-356, CVC-968, and CVC-12K.}
    \label{table:results2}
   \def\arraystretch{1.1}
    \setlength\tabcolsep{5pt}
    \par\bigskip
    \centering
        \resizebox{\columnwidth}{!}{%
           \begin{tabular}{ l c c c c } 
                \bottomrule
                Method & DICE & IoU & Recall & Precision\\ 
                  \toprule
                \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-356}} \\
              \bottomrule
                ResUNet++ & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline
                {ResUNet++ + CRF} & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline
                {ResUNet++ + TTA} & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline
                {ResUNet++ + CRF + TTA} & 0.0000  & 0.0000 & 0.0000 & 0.0000\\ % \hline
                \toprule
                \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-612}}\\
              \bottomrule
              ResUNet++& 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline  
              {ResUNet++ + CRF} & 0.0000 & 0.0000  & 0.0000 & 0.0000\\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  & 0.0000 & 0.0000\\ % \hline
              {ResUNet++ + CRF + TTA} & 0.0000  & 0.0000 & 0.0000 & 0.0000 \\ % \hline
                \toprule  
             \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-968}} \\
              \bottomrule
              ResUNet++& 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline  
              {ResUNet++ + CRF} & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  &  0.0000 & 0.0000\\ % \hline
              {ResUNet++ + CRF + TTA} & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline
                \toprule  
                \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = CVC-12K}} \\
              \bottomrule
              {ResUNet++}& 0.0000 & 0.0000 & 0.0000  & 0.0000 \\ % \hline  
              {ResUNet++ + CRF} & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ % \hline
              {ResUNet++ + CRF + TTA} & 0.0000 & 0.0000 & 0.0000  & 0.0000 \\ % \hline
                \toprule 
             \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = Kvasir-SEG}} \\
              \bottomrule
              ResUNet++ &  0.0000 & 0.0000  & 0.0000  & 0.0000 \\ % \hline  
              {ResUNet++ + CRF}& 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline
              {ResUNet++ + CRF + TTA} & 0.0000  & 0.0000 & 0.0000  & 0.0000 \\ % \hline
                \toprule 
            \multicolumn{5}{c}{\textbf{Model Train = ETIS-LARIB, Test = Colon-DB}} \\
              \bottomrule
              ResUNet++ &  0.0000 & 0.0000  & 0.0000  & 0.0000 \\ % \hline  
              {ResUNet++ + CRF}& 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline 
              {ResUNet++ + TTA} & 0.0000 & 0.0000  & 0.0000 & 0.0000 \\ % \hline
              {ResUNet++ + CRF + TTA} & 0.0000  & 0.0000 & 0.0000  & 0.0000 \\ % \hline
                \toprule 
\end{tabular}}
\end{table}						



==> results_on_same_dataset.tex <==
%=======================Kvasir-SEG==================================================
\begin{table}[!t]
 \caption{Result comparison on Kvasir-SEG}
    \label{table:resultkvasir}
   %\def\arraystretch{1.1}
    % \setlength\tabcolsep{5pt}
\scriptsize
    \centering
        %\resizebox{\columnwidth}{!}{%
           \begin{tabular}{ l c c c c} 
                \toprule
                Method & DSC & mIoU & Recall & Precision\\ 
              \bottomrule
                 UNet~\cite{ronneberger2015u} & 0.7147 & 0.4334 & 0.6306 & \textbf{0.9222} \\
                 ResUNet~\cite{zhang2018road} & 0.5144 & 0.4364  & 0.5041 & 0.7292 \\ 
                 ResUNet-mod~\cite{zhang2018road} & 0.7909 & 0.4287 & 0.6909 & 0.8713 \\ 
                 \resunetplusplus~\cite{jha2019resunet++} & 0.8119  & 0.8068 & 0.8578 & 0.7742\\ 
                 \resunetplusplus + CRF & 0.8129 & 0.8080 & 0.8574 & 0.7775\\ 
                 \resunetplusplus TTA & 0.8496 & 0.8318 & \textbf{0.8760} & 0.8203\\
                 \resunetplusplus +TTA + CRF  & \textbf{0.8508} & \textbf{0.8329} & 0.8756 &0.8228\\
               \bottomrule
\end{tabular}%}
     \vspace{-3mm} 
\end{table}						


%=======================CVC-612==================================================
\begin{table}[!t]
 \caption{Result comparison on CVC-ClinicDB}
    \label{table:resultcvc612}
   %\def\arraystretch{1.1}
    %\setlength\tabcolsep{5pt}
    \scriptsize
    \centering
       % \resizebox{\columnwidth}{!}{%
           \begin{tabular}{ l c c c c} 
                \toprule
                Method & DSC & mIoU & Recall & Precision\\ 
              \bottomrule
                MultiResUNet$^\diamond$~\cite{ibtehaz2020multiresunet}&  - & 0.8497 & - & -\\
                cGAN$^\dag$~\cite{poomeshwaran2019polyp} & 0.8848 & 0.8127 & - & -\\ 
                SegNet\cite{wang2018development} & - & - & 0.8824 & -\\ 
                FCN$^\bullet$~\cite{li2017colorectal} & - &- &0.7732 & \textbf{0.8999}\\ 
                CNN~\cite{nguyen2018colorectal} & (0.62-0.87) &- &- & -\\
                {MSPB$^\psi$~CNN}~\cite{banik2020multi} & 0.8130 &- &0.7860 & 0.8090\\
                UNet~\cite{ronneberger2015u} &  0.6419 & 0.4711 & 0.6756 & 0.6868 \\ 
               ResUNet~\cite{zhang2018road} & 0.4510 & 0.4570 & 0.5775 & 0.5614 \\
                {PraNet~\cite{fan2020pranet}} & 0.8980 &0.8400 & - & - \\
                
                ResUNet-mod~\cite{zhang2018road} & 0.7788 & 0.4545 & 0.6683 & 0.8877\\ 
               \resunetplusplus~\cite{jha2019resunet++} & 0.9199 & 0.8892 & 0.9391 & 0.8445 \\ 
                \resunetplusplus + \ac{CRF}  & \textbf{0.9203} & \textbf{0.8898} & \textbf{0.9393} & 0.8459\\ 
                \resunetplusplus + \ac{TTA} & 0.9020 & 0.8826 & 0.9065 & 0.8539 \\
                \resunetplusplus + \ac{TTA} + \ac{CRF} & 0.9017 & 0.8828 & 0.9060 & 0.8549\\
                 \bottomrule
                \multicolumn{4}{l}{$^\dag$ Conditional generative adversarial network} \hspace{.1cm} $^\diamond${Data augmentation}\\
	   \multicolumn{4}{l}{$^\bullet$Fully convolutional network \hspace{.1cm} {$^\psi$ multi-scale patch-based}}
\end{tabular}%}
 \vspace{-3mm} 
\end{table}						
%=======================CVC-ColonDB==================================================

\begin{table}[!t]
 \caption{Results comparison on CVC-ColonDB}
 %[lr=1e-4, batch size = 16, loss = binary_crossentropy, Optimizer = Nadam, ]
    \label{table:resultCVC-ColonDB}
%   \def\arraystretch{1.1}
%     \setlength\tabcolsep{5pt}
\scriptsize
    \centering
        %\resizebox{\columnwidth}{!}{%
           \begin{tabular}{ l c c c c c } 
                \toprule
                Method & DSC & \ac{mIoU} & Recall & Precision\\ 
              \bottomrule
                {FCN-8S + Otsu}~\cite{akbari2018polyp} & 0.8100 & - &0.7480 & -\\ 
                {FCN-8s + Texton}~\cite{zhang2017automated} & 0.7014 & - &0.7566 &-\\
                {SA-DOVA Descriptor}~\cite{bernal2012towards}& 0.5533& -& 0.6191& -\\
                {PraNet~\cite{fan2020pranet}} & 0.7090 & 0.6400 & - & - \\
                
                \resunetplusplus~\cite{jha2019resunet++}& 0.8469 &0.8456 &\textbf{0.8511} &0.8003  \\
                {\resunetplusplus + CRF}& 0.8458 &0.8456 &0.8497 &0.7767\\ % 
                {\resunetplusplus + TTA}& \textbf{0.8474} &\textbf{0.8466} &0.8434 &0.8118\\ %
                {\resunetplusplus + TTA + CRF}&0.8452 &0.8459 &0.8411 &\textbf{0.8125}\\ 
                \bottomrule
                  \vspace{-5mm} 
\end{tabular}%}
\end{table}						

%=======================ETIS-Larib_comparision==================================
\begin{table}[!t]
 \caption{Results on ETIS-Larib Polyp DB} 
 %final results lr =1e-5, 300 epoch, 247 epoch (converged)
    \label{table:resultetislarib}
   %\def\arraystretch{1.1}
    %\setlength\tabcolsep{5pt}
    \scriptsize
    \centering
        %\resizebox{\columnwidth}{!}{%
           \begin{tabular}{l c c c c c} 
                \toprule
                Method & DSC & \ac{mIoU} & Recall & Precision\\ 
              \bottomrule
                ResUNet++~\cite{jha2019resunet++} &\textbf{0.6364} &\textbf{0.7534} &\textbf{0.6346} &0.6467\\
                {PraNet~\cite{fan2020pranet}} & 0.6280 & 0.5670 & - & - \\
                {ResUNet++ + CRF} &0.6228 &0.7520 &0.6242 &0.5648\\
                {ResUNet++ + TTA}&0.6136  &0.7458 &0.5996 &\textbf{0.6565}\\ 
                {ResUNet++ + TTA + CRF}&0.6018 &0.7426 &0.5914 &0.5755\\ 
                \bottomrule
                 \vspace{-5mm} 
\end{tabular}%}
\end{table}						



\begin{table}[t!]
 \caption{Results comparison on CVC-VideoClinicDB}
 %[lr=1e-4, batch size = 16, loss = binary_crossentropy, Optimizer = Nadam,]
    \label{table:CVC-VideoClinicDB}
   %\def\arraystretch{1.1}
    %\setlength\tabcolsep{5pt}
    \scriptsize
    \centering
        %\resizebox{\columnwidth}{!}{%
           \begin{tabular}{ l c c c c c } 
                \toprule
                Method & DSC & \ac{mIoU} & Recall & Precision\\ 
              \bottomrule
                \resunetplusplus~\cite{jha2019resunet++} &0.8798 &0.8730 &\textbf{0.7749} &0.6702 \\
                {\resunetplusplus + CRF} &\textbf{0.8811} &\textbf{0.8739} &0.7743 &\textbf{0.6706}\\ % 
                {\resunetplusplus + TTA} &0.8125 &0.8467 &0.6896 &0.6421\\ %
                {\resunetplusplus + TTA + CRF} &0.8130 &0.8477 &0.6875 &0.6276\\ 
                \bottomrule
\end{tabular}%}
 \vspace{-3mm} 
\end{table}						



				

\begin{table}[t!]
 \caption{Results comparison on ASUMayo Clinic}
 %[lr=1e-4, batch size = 16, loss = binary_crossentropy, Optimizer = Nadam, ]
    \label{table:ASUMayo}
   %\def\arraystretch{1.1}
    %\setlength\tabcolsep{5pt}
\scriptsize
    \centering
        %\resizebox{\columnwidth}{!}{%

           \begin{tabular}{ l c c c c c } 
                \toprule
                Method & DSC & \ac{mIoU} & Recall & Precision\\ 
              \bottomrule
                \resunetplusplus~\cite{jha2019resunet++} &0.8743 &0.8569 &\textbf{0.6534}  &0.4896    \\
                {\resunetplusplus + CRF} &\textbf{0.8850}  &\textbf{0.8635} &0.6504 &0.4858    \\ % 
                {\resunetplusplus + TTA} &0.8553 &0.8535    &0.6162 &\textbf{0.4912} \\ %
                {\resunetplusplus + TTA + CRF} &0.8550 &0.8551 &0.6107 &0.4743    \\ 
                \bottomrule
\end{tabular}%}
 \vspace{-3mm} 
\end{table}						


\begin{table}[t!]
 \caption{Results comparison on mixed dataset}
 %[lr=1e-4, batch size = 16, loss = binary_crossentropy, Optimizer = Nadam, ]
    \label{table:mixeddataset}
  %\def\arraystretch{1.1}
    %\setlength\tabcolsep{5pt}
    \scriptsize
    \centering
        %\resizebox{\columnwidth}{!}{%
          \begin{tabular}{ l c c c c c } 
 
                \toprule
                Method & DSC & \ac{mIoU} & Recall & Precision\\ 
                \bottomrule

                \multicolumn{5}{c}{\textbf{Model Train = (Kvasir-SEG + CVC-ClinicDB), Test = CVCColonDB}}\\
              \bottomrule
                \resunetplusplus~\cite{jha2019resunet++} &0.4974 &0.6800 & 0.4787  &\textbf{0.6019}    \\
                {\resunetplusplus + CRF} & 0.4920 &0.6788 &0.4744 &0.5636   \\ % 
                {\resunetplusplus + TTA} & \textbf{0.5084} &\textbf{0.6859} &\textbf{0.4795} &0.5973   \\ %
                {\resunetplusplus + TTA + CRF}&0.5061  &0.6852 &0.4775 &0.5770\\ 
                \bottomrule
                \multicolumn{5}{c}{\textbf{Model Train = (Kvasir-SEG + CVC-ClinicDB), Test =  CVCVideoClinicDB}}\\
              \bottomrule
                \resunetplusplus~\cite{jha2019resunet++} &0.3460 & 0.6348 & \textbf{0.2272}  & \textbf{0.3383}\\
                {\resunetplusplus + CRF} & 0.3552 & 0.6412 & 0.2228 & 0.3065\\ % 
                {\resunetplusplus + TTA} & 0.3573 & 0.6440 & 0.2104 & 0.3338 \\ %
                {\resunetplusplus + TTA + CRF}& \textbf{0.3603} & \textbf{0.6468} & 0.2068 & 0.3038 \\ 
                \bottomrule 
\end{tabular}%}
 \vspace{-3mm} 
\end{table}
